The Electric Field Dependence of Single Electron Emission in the PIXeY Two-Phase Xenon Detector

Dual phase xenon detectors are widely used in experimental searches for galactic darkmatter particles. The origin of single electron backgrounds following prompt scintillation and proportional scintillation signals in these detectors is not fully understood, although there has been progress in recent years. In this paper, we describe single electron backgrounds in ${}^{83m}Kr$ calibration events and their correlation with drift and extraction fields, using the Particle Identification in Xenon at Yale (PIXeY) dual-phase xenon time projection chamber. The single electron background induced by the Fowler-Nordheim (FN) effect is measured, and its electric field dependence is quantified. The photoionization of grids and impurities by prompt scintillation and proportional scintillation also contributes to the single electron background.

==> arxiv version/bib.tex <==
\begin{thebibliography}{100}

\bibitem{luxKr} LUX Collaboration, D.S. Akerib et. al., \emph{$\mathrm{^{83m}Kr}$ calibration of the 2013 LUX dark matter search, Phys. Rev. D} {\bf 96} (2017) \href{https://arxiv.org/pdf/1708.02566.pdf}{[arxiv:1708.02566]}

\bibitem{Boulton} E. M. Boulton and E. Bernard and N. Destefano and B. N. V. Edwards and M. Gai and S. A. Hertel and M. Horn and N. A. Larsen and B. P. Tennyson and C. Wahl and D. N. McKinsey.\emph{Calibration of a two-phase xenon time projection chamber with a $^{37}$Ar source.} JINST 12 (2017) 08, P08004 \href{https://arxiv.org/pdf/1705.08958.pdf}{[arXiv:1705.08958]} .

\bibitem{Santos} E. Santos \textit{et. al.} ZEPLIN-III Collaboration \emph{Single electron emission in two-phase xenon with application to the detection of coherent neutrino-nucleus scattering.} JHEP 1112. 115 (2011) 112009. \href{https://arxiv.org/abs/1110.3056}{[arXiv:1110.3056]}

\bibitem{Angle} E. Angle \textit{et. al.} XENON10 Collaboration\emph{A search for light dark matter in XENON10 data} Phys.Rev. 107:051301 (2011) \href{https://arxiv.org/abs/1104.3088}{[arXiv:1104.3088]}

\bibitem{Sorensen} P. F. Sorensen, K. J. Kamdin. \emph{Two distinct components of the delayed single electron background signals in liquid xenon emission detectors} {\bf 96} JINST 13 (2018). \href{https://arxiv.org/pdf/1711.07025v2.pdf}{[arXiv:1711.07025v2]}

\bibitem{Edwards} B.Edwards \textit{et. al.} \emph{Measurement of single electron emission in two-phase xenon.} \textit{Astropart.Phys}. 30 (2008) 54-57 \href{https://inspirehep.net/literature/757633}{[doi:10.1016/j.astropartphys.2008.06.006]}

\bibitem{Aprile} E Aprile et al. [XENON100 Collaboration]. \emph{Observation and applications of single-electron charge signals in the XENON100 experiment, J. Phys. G: Nucl. Part. Phys. 41 (2014) 035201} \href{https://arxiv.org/abs/1311.1088}{[arXiv:1311.1088]}

\bibitem{Bailey} A. Bailey, \emph{Dark Matter Searches and Study of Electrode Design in LUX and LZ, Ph.D. thesis, Imperial College London} (2016) \href{https://www.semanticscholar.org/paper/Dark-matter-searches-and-study-of-electrode-design-Bailey/5c997b8a790e57bf5efec0ce40aa15db6fe7e629}{[PDF]}.

\bibitem{Nordheim} L. W. Nordheim, \emph{“The effect of the image force on the emission and reflection of electrons by metals,”} Proc. R Soc. London A, 121 788, 626–639 (1928)

\bibitem{grids} Tomás, A., Araújo, H.M., \textit{et. al.}  \emph{Study and mitigation of spurious electron emission from cathodic wires in noble liquid time projection chambers.} \textit{ Astroparticle Physics} 103 (2018): 49-61. \href{https://arxiv.org/abs/1801.07231}{[arXiv:1801.07231]}

\bibitem{Alpert} Alpert, D., Lee, D. A., Lyman, E. M., Tomaschke, H. E. (1964). Initiation of Electrical Breakdown in Ultrahigh Vacuum. Journal of Vacuum Science and Technology, 1(2), 35–50. \href{https://avs.scitation.org/doi/10.1116/1.1491722}{[doi:10.1116]}

\bibitem{Malter} L.~Malter, \emph{Thin Film Field Emission, Phys. Rev.} {\bf 50} (1936) 48. \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.50.48}{PhysRev.50.48}

\bibitem{Akimov} D.Yu. Akimov, et al. 2016 \emph{Observation of delayed electron emission in a two- phase liquid xenon detector} JINST 11 C03007 \href{https://iopscience.iop.org/article/10.1088/1748-0221/11/03/C03007/pdf}{[PDF]}

\bibitem{edwards_eff} B.N.V Edwards \textit{et. al.}, \emph{Extraction efficiency of drifting electrons in a two-phase
xenon time projection chamber, JINST} {\bf 13} (2018) \href{https://arxiv.org/pdf/1710.11032.pdf}{[arxiv:1710.11032]}

\bibitem{Anisha} A. G. Singh, \textit{et. al.} \emph{Calibration of a Liquid Xenon Detector with \ce{^{83m}_{}Kr}, Phys.Rev.C.} {\bf 80} (2009) 045809 \href{https://arxiv.org/pdf/0905.1766.pdf}{[arXiv:0905.1766]}

\bibitem{evan} N. E. Destefano, \emph{Design, Construction, and Optimization of the Energy Resolution of a Xenon TPC Detector} (Doctoral Dissertation) opencommons.uconn.edu (2015) \href{https://opencommons.uconn.edu/cgi/viewcontent.cgi?article=7228&context=dissertations}{[PDF]}

\bibitem{ks} L. W. Kastens, S. B. Cahn, A. Manzur, and D. N. McKinsey, \emph{Calibration of a Liquid Xenon Detector with \ce{^{83m}_{}Kr}, Phys.Rev.C.} {\bf 80} (2009) 045809 \href{https://arxiv.org/pdf/0905.1766.pdf}{[arXiv:0905.1766]}

\bibitem{Larsen} N.A. Larsen. \emph{Two-Phase Xenon Time Projection Chambers for WIMP Searches and Other Applications, Thesis} (2015).

\bibitem{Noer} Noer, R.J. \emph{Electron field emission from broad-area electrodes.} Appl. Phys. A 28, 1–24 (1982)  \href{https://link.springer.com/article/10.1007/BF00617778}{[doi:10.1007]}

\bibitem{Zhou} Y. Zhou, P. Zhang \emph{A quantum model for photoemission from metal surfaces and its comparison with the three-step model and Fowler–DuBridge model,J. Appl. Phys. 127}  (2020) 164903 \href{https://doi.org/10.1063/5.0004140}{[doi:10.1063]}



\bibitem{Aprile:2014} E.~Aprile \textit{et. al.} \emph{Measurements of proportional scintillation and electron multiplication in liquid xenon using thin wires, JINST} {\bf 9} (2014) P11012.\href{https://arxiv.org/abs/1408.6206}{arXiv:1408.6206}

\bibitem{MicroBooNE} R. Acciarri \textit{et. al.} \emph{Liquid argon dielectric breakdown studies with the MicroBooNE purification system, JINST} {\bf 9} (2014) P11001 \href{https://iopscience.iop.org/article/10.1088/1748-0221/9/11/P11001}{[doi:10.1088/1748- 0221/9/11/P11001.]}{[arXiv:1908.06888]}

\bibitem{XeBrA} L.~Tvrznikova \textit{et. al.} \emph{Direct comparison of high voltage breakdown measurements in liquid argon and liquid xenon, JINST} {\bf 14} (2019) P12018 \href{https://iopscience.iop.org/article/10.1088/1748-0221/14/12/P12018}{arXiv:1908.06888}

\bibitem{F-hypothesis} R. Fowler, \emph{Statistical Mechanics.} \textit{Cambridge University Press}, London,
1936, p. 355.

\bibitem{Sodha} M. S. Sodha, A. Dixit, and S. Srivastava. \emph{Photoelectric field emission of electrons: Photon assisted tunneling} \textit{Appl. Phys. Lett.} 94, 251501 (2009);
\href{https://doi.org/10.1063/1.3158595}{https://doi.org/10.1063/1.3158595}

\bibitem{Forbes_2} R. G. Forbes, \emph{Journal of Vacuum Science and Technology B: Microelectronics and Nanometer Structures Processing},
\textit{Measurement, and Phenomena} 26, 788 (2008)
\href{https://avs.scitation.org/doi/pdf/10.1116/1.2827505}{[doi: 10.1116/1.2827505]}

\bibitem{Brodie} I. Brodie \emph{Studies of Field Emission and Electrical Breakdown Between Extended Nickel Surfaces in Vacuum} \textit{Journal of Applied Physics} 35, 2324 (1964)
\href{https://doi.org/10.1063/1.1702858}{[doi:10.1063]}

\bibitem{Jingke} D. S. Akerib, \textit{et. al.}, \emph{Investigation of background electron emission in the LUX detector} (2020) \href{https://arxiv.org/abs/2004.07791}{[arXiv:2004.07791]}



\bibitem{Cox} Cox, B. M., Williams, W. T. (1977). \emph{Field-emission sites on unpolished stainless steel}. Journal of Physics D: Applied Physics, 10(3), L5–L9.\href{doi:10.1088/0022-3727/10/3/001}{[doi:10.1088]}

\bibitem{princeton} Kirk T. McDonald \emph{Notes on Electrostatic Wire Grids}. Joseph Henry Laboratories, Princeton University, Princeton, NJ 08544. (2003) \href{https://www.researchgate.net/publication/246980598_Notes_on_Electrostatic_Wire_Grids}{[PDF]}

\bibitem{Williams} Williams, D. W., Williams, W. T. \emph{Field-emitted current necessary for cathode-initiated vacuum breakdown.} Journal of Physics D: Applied Physics, 5(2), 280–290. (1972) \href{ doi:10.1088/0022-3727/5/2/309 1972.}{[doi:10.1088]}

\bibitem{Forbes} Forbes Richard G. and Deane Jonathan H. B. \emph{Transmission coefficients for the exact triangular barrier: an exact general analytical theory that can replace Fowler- Nordheim's 1928 theory} Proc. R. Soc. A.4672927–2947, (2011)\href{https://royalsocietypublishing.org/doi/full/10.1098/rspa.2011.0025}{[doi: 2011.0025]}

\bibitem{smith} Little, R. P., Smith, S. T. .\emph{Field Enhancing Projections Produced by the Application of an Electric Field.} Journal of Applied Physics, 36(4), 1502–1504. (1965) \href{https://aip.scitation.org/doi/10.1063/1.1714350}{[doi:10.1063]}

\bibitem{Keiko} Keiko Fujii, \textit{et. al.} \emph{High-accuracy measurement of the emission spectrum of liquid xenon in the vacuum ultraviolet region} {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment, Volume 795, 21 September, Pages 293-297} (2015) \href{https://doi.org/10.1016/j.nima.2015.05.065}{[doi:10.1016]}

\bibitem{QE} E.Aprile \textit{et. al.} \emph{Performance of Dual Phase XeTPC with CsI Photocathode and PMTs readout for the
Scintillation Light} \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=1490096&tag=1}{[PDF]}

\bibitem{pmt} \emph{Photomultiplier Tubes
Basics and Applications} HAMAMATSU PHOTONICS K. K. (2007) \href{https://www.hamamatsu.com/resources/pdf/etd/PMT_handbook_v3aE.pdf}{[PDF]}


\end{thebibliography}

%%%%% CLEAR DOUBLE PAGE!
\newpage{\pagestyle{empty}\cleardoublepage}
